Rigid Surface Operators

Surface operators in gauge theory are analogous to Wilson and 't Hooft line operators except that they are supported on a two-dimensional surface rather than a one-dimensional curve. In a previous paper, we constructed a certain class of half-BPS surface operators in N=4 super Yang-Mills theory, and determined how they transform under S-duality. Those surface operators depend on a relatively large number of freely adjustable parameters. In the present paper, we consider the opposite case of half-BPS surface operators that are ``rigid'' in the sense that they do not depend on any parameters at all. We present some simple constructions of rigid half-BPS surface operators and attempt to determine how they transform under duality. This attempt is only partially successful, suggesting that our constructions are not the whole story. The partial match suggests interesting connections with quantization. We discuss some possible refinements and some string theory constructions which might lead to a more complete picture.

==> toc.tex <==
\noindent {1.} {Introduction} \leaderfill{1} \par 
\noindent {2.} {Rigid Surface Operators} \leaderfill{4} \par 
\noindent \quad{2.1.} {Review} \leaderfill{4} \par 
\noindent \quad{2.2.} {Limit For $\alpha ,\beta ,\gamma \to 0$} \leaderfill{7} \par 
\noindent \quad{2.3.} {Searching For Rigid Surface Operators} \leaderfill{14} \par 
\noindent \quad{2.4.} {Strongly Rigid Semisimple Orbits} \leaderfill{21} \par 
\noindent \quad{2.5.} {Combining The Two Constructions} \leaderfill{27} \par 
\noindent {3.} {Alternative Point of View} \leaderfill{29} \par 
\noindent \quad{3.1.} {Coupling To Sigma Models} \leaderfill{29} \par 
\noindent \quad{3.2.} {An Example} \leaderfill{31} \par 
\noindent \quad{3.3.} {Another Example} \leaderfill{33} \par 
\noindent \quad{3.4.} {Rigid Surface Operator For The Dual Group} \leaderfill{37} \par 
\noindent \quad{3.5.} {Minimal Surface Operators} \leaderfill{40} \par 
\noindent {4.} {Fingerprints of Surface Operators} \leaderfill{41} \par 
\noindent \quad{4.1.} {Invariant Polynomials} \leaderfill{41} \par 
\noindent \quad{4.2.} {Polar Polynomials} \leaderfill{43} \par 
\noindent \quad{4.3.} {Center vs. Topology} \leaderfill{50} \par 
\noindent {5.} {Duality for Strongly Rigid Surface Operators} \leaderfill{53} \par 
\noindent \quad{5.1.} {Duality for $G = SO(5)$ and ${^L\kern -.16667em G}= Sp(4)$} \leaderfill{53} \par 
\noindent \quad{5.2.} {Duality for $G = SO(8)$} \leaderfill{56} \par 
\noindent \quad{5.3.} {Duality for $G = SO(7)$ and ${^L\kern -.16667em G}= Sp(6)$} \leaderfill{57} \par 
\noindent \quad{5.4.} {Duality for $G = SO(9)$ and ${^L\kern -.16667em G}= Sp(8)$} \leaderfill{58} \par 
\noindent {6.} {More Examples} \leaderfill{60} \par 
\noindent \quad{6.1.} {Special Rigid Orbits} \leaderfill{60} \par 
\noindent \quad{6.2.} {Dualities Involving Rigid Semisimple Orbits} \leaderfill{66} \par 
\noindent {7.} {Duality and Quantization} \leaderfill{67} \par 
\noindent {8.} {Stringy Constructions of Rigid Surface Operators} \leaderfill{71} \par 
\noindent \quad{8.1.} {Holographic Description} \leaderfill{71} \par 
\noindent \quad{8.2.} {Application: $SO(2N)$ Gauge Theory} \leaderfill{73} \par 
\noindent \quad{8.3.} {Intersecting Brane Models} \leaderfill{75} \par 
\noindent \quad{8.4.} {Bubbling Geometries} \leaderfill{77} \par 
\noindent Appendix {A.} {Rigid Nilpotent Orbits for Exceptional Groups} \leaderfill{80} \par 
\noindent Appendix {B.} {Orthogonal and Symplectic Lie Algebras and Duality} \leaderfill{83} \par 

